Phase diagram of a lattice fermion model with symmetric mass generation

We study the phase structure of a model containing two flavors of massless staggered fermions interacting through two independent four-fermion couplings, UI and UB, formulated on a three-dimensional Euclidean space-time lattice. At UB = 0, this model is known to exhibit a direct second-order quantum phase transition between a massless fermion (MF) phase and a phase in which fermions acquire masses through the mechanism commonly referred to as symmetric mass generation (SMG). We demonstrate that introducing a small nonzero value of UB qualitatively alters this structure: the single exotic transition at UB = 0 splits into two distinct, conventional transitions, separated by an intermediate phase in which fermion masses arise through the standard mechanism of spontaneous symmetry breaking (SSB). The first of these is a Gross-Neveu transition separating the MF phase from the SSB-induced massive phase, while the second is a three-dimensional XY transition between the SSB phase and the SMG phase. Using the fermion-bag Monte Carlo method, we verify that the critical exponents associated with both transitions are consistent with the literature, thereby yielding a quantitative characterization of the resulting phase structure of the model.

==> header-1-packages.tex <==
\ifx\pdfsuppresswarningpagegroup\undefined\else\pdfsuppresswarningpagegroup=1\fi\relax
\RequirePackage{silence}
\WarningFilter{nameref}{The definition of \label has changed!}
\WarningFilter{revtex4-2}{Repair the float package}
\PassOptionsToPackage{unicode, pdfprintscaling=None, colorlinks}{hyperref}

\usepackage{hyperref}
\usepackage{orcidlink,multirow,siunitx,colortbl,dcolumn,tikz,graphicx,latexsym,amsmath,amssymb,amsfonts,bm,bbm,microtype,xspace,placeins,float,mathtools,xcolor,makecell,tabularx}

\usepackage[normalem]{ulem}
\usepackage[export]{adjustbox}
\usepackage[capitalise]{cleveref}

\usetikzlibrary{decorations.markings, arrows, decorations.pathmorphing}
\graphicspath{{pic/}}

\allowdisplaybreaks
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newlength{\FigureWidth}
\setlength{\FigureWidth}{3.3in}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\newcommand\TopRule{\Xhline{0.08em}}
\newcommand\HeaderRule{\Xhline{0.05em}}
\newcommand\MidRule{\Xhline{0.03em}}
\newcommand\BotRule{\Xhline{0.08em}}
\newcommand\SetTableProperties{
  \renewcommand{\arraystretch}{1.4}
}

\WarningFilter{revtex4-2}{Deferred float stuck}
\WarningFilter{latex}{A float is stuck}

\makeatletter
\newcommand\showtitleinbib{{\escapechar=`\\ \immediate\write\@auxout{%
\csname citation{REVTEX42Control}\endcsname^^J%
\csname citation{apsrev42Control}\endcsname
}}}
\makeatother


==> header-6-main.tex <==













